The Polynomial Set Associated with a Fixed Number of Matrix-Matrix Multiplications

We consider the problem of computing matrix polynomials $p(X)$, where $X$ is a large dense matrix, with as few matrix-matrix multiplications as possible. More precisely, let $\Pi_{2^{m}}^*$ represent the set of polynomials computable with $m$ matrix-matrix multiplications, but with an arbitrary number of matrix additions and scaling operations. We characterize this set through a tabular parameterization. By deriving equivalence transformations of the tabular representation, we establish new methods that can be used to construct elements of $\Pi_{2^{m}}^*$ and determine general properties of the set. The transformations allow us to eliminate variables and prove that the dimension is bounded by $m^2$, which is subsequently proven to be sharp, i.e., $\dim(\Pi_{2^m}^*)=m^2$. Consequently, we have identified a parameterization that, to the best of our knowledge, is the first minimal parameterization. We also conduct a study using computational tools from algebraic geometry to determine the largest degree $d$ such that all polynomials of that degree belong to $\Pi_{2^{m}}^*$, or its closure. In many cases, the computational setup is constructive in the sense that it can also be used to determine a specific evaluation scheme for a given polynomial.

==> gfx/reduced_data.tex <==
\pgfmathsetmacro{\baseoffset}{-0.1} % Define the base offset
\addplot+[only marks, mark=o]
    coordinates {
        (3, 8)
        (4, 16)
        (5, 32)
        (6, 64)
        (7, 128)
    };
\addlegendentry{0 reductions}

\pgfmathsetmacro{\offset}{1*\baseoffset}  % Reduction=1
\addplot+[only marks, mark=+]
    coordinates {
        (3-\offset, 6)
        (4-\offset, 12)
        (5-\offset, 24)
        (6-\offset, 48)
        (7-\offset, 96)
    };
\addlegendentry{1 reductions}
\pgfmathsetmacro{\offset}{2*\baseoffset}  % Reduction=2
\addplot+[only marks, mark=x]
    coordinates {
        (3-\offset, 5)
        (3-\offset, 4)
        (4-\offset, 10)
        (4-\offset, 9)
        (4-\offset, 8)
        (5-\offset, 20)
        (5-\offset, 18)
        (5-\offset, 16)
        (6-\offset, 40)
        (6-\offset, 36)
        (6-\offset, 32)
        (7-\offset, 80)
        (7-\offset, 72)
        (7-\offset, 64)
    };
\addlegendentry{2 reductions}
\pgfmathsetmacro{\offset}{3*\baseoffset}  % Reduction=3
\addplot+[only marks, mark=triangle]
    coordinates {
        (3-\offset, 4)
        (3-\offset, 3)
        (4-\offset, 8)
        (4-\offset, 6)
        (4-\offset, 9)
        (5-\offset, 16)
        (5-\offset, 15)
        (5-\offset, 12)
        (5-\offset, 18)
        (6-\offset, 32)
        (6-\offset, 30)
        (6-\offset, 27)
        (6-\offset, 24)
        (6-\offset, 36)
        (7-\offset, 64)
        (7-\offset, 60)
        (7-\offset, 54)
        (7-\offset, 48)
        (7-\offset, 72)
    };
\addlegendentry{3 reductions}
\pgfmathsetmacro{\offset}{4*\baseoffset}  % Reduction=4
\addplot+[only marks, mark=diamond]
    coordinates {
        (3-\offset, 3)
        (3-\offset, 4)
        (3-\offset, 2)
        (4-\offset, 7)
        (4-\offset, 6)
        (4-\offset, 8)
        (4-\offset, 5)
        (4-\offset, 4)
        (5-\offset, 14)
        (5-\offset, 12)
        (5-\offset, 13)
        (5-\offset, 10)
        (5-\offset, 16)
        (5-\offset, 8)
        (5-\offset, 9)
        (5-\offset, 17)
        (6-\offset, 28)
        (6-\offset, 24)
        (6-\offset, 26)
        (6-\offset, 25)
        (6-\offset, 20)
        (6-\offset, 32)
        (6-\offset, 18)
        (6-\offset, 16)
        (6-\offset, 27)
        (6-\offset, 34)
        (7-\offset, 56)
        (7-\offset, 48)
        (7-\offset, 52)
        (7-\offset, 50)
        (7-\offset, 45)
        (7-\offset, 40)
        (7-\offset, 64)
        (7-\offset, 36)
        (7-\offset, 32)
        (7-\offset, 54)
        (7-\offset, 68)
    };
\addlegendentry{4 reductions}
\pgfmathsetmacro{\offset}{5*\baseoffset}  % Reduction=5
\addplot+[only marks, mark=pentagon]
    coordinates {
        (3-\offset, 3)
        (3-\offset, 2)
        (4-\offset, 6)
        (4-\offset, 5)
        (4-\offset, 4)
        (4-\offset, 8)
        (4-\offset, 3)
        (5-\offset, 12)
        (5-\offset, 11)
        (5-\offset, 10)
        (5-\offset, 9)
        (5-\offset, 8)
        (5-\offset, 13)
        (5-\offset, 6)
        (5-\offset, 16)
        (6-\offset, 24)
        (6-\offset, 22)
        (6-\offset, 21)
        (6-\offset, 20)
        (6-\offset, 18)
        (6-\offset, 16)
        (6-\offset, 23)
        (6-\offset, 15)
        (6-\offset, 26)
        (6-\offset, 12)
        (6-\offset, 32)
        (6-\offset, 33)
        (7-\offset, 48)
        (7-\offset, 44)
        (7-\offset, 42)
        (7-\offset, 40)
        (7-\offset, 36)
        (7-\offset, 32)
        (7-\offset, 39)
        (7-\offset, 46)
        (7-\offset, 30)
        (7-\offset, 45)
        (7-\offset, 52)
        (7-\offset, 24)
        (7-\offset, 27)
        (7-\offset, 51)
        (7-\offset, 64)
        (7-\offset, 66)
    };
\addlegendentry{5 reductions}
\pgfmathsetmacro{\offset}{6*\baseoffset}  % Reduction=6
\addplot+[only marks, mark=star]
    coordinates {
        (3-\offset, 2)
        (4-\offset, 5)
        (4-\offset, 4)
        (4-\offset, 6)
        (4-\offset, 3)
        (4-\offset, 8)
        (4-\offset, 2)
        (5-\offset, 10)
        (5-\offset, 8)
        (5-\offset, 9)
        (5-\offset, 12)
        (5-\offset, 7)
        (5-\offset, 6)
        (5-\offset, 11)
        (5-\offset, 5)
        (5-\offset, 4)
        (5-\offset, 16)
        (6-\offset, 20)
        (6-\offset, 18)
        (6-\offset, 16)
        (6-\offset, 15)
        (6-\offset, 14)
        (6-\offset, 24)
        (6-\offset, 19)
        (6-\offset, 12)
        (6-\offset, 22)
        (6-\offset, 17)
        (6-\offset, 13)
        (6-\offset, 10)
        (6-\offset, 8)
        (6-\offset, 25)
        (6-\offset, 9)
        (6-\offset, 21)
        (6-\offset, 32)
        (7-\offset, 40)
        (7-\offset, 36)
        (7-\offset, 33)
        (7-\offset, 32)
        (7-\offset, 35)
        (7-\offset, 30)
        (7-\offset, 28)
        (7-\offset, 48)
        (7-\offset, 38)
        (7-\offset, 27)
        (7-\offset, 24)
        (7-\offset, 44)
        (7-\offset, 34)
        (7-\offset, 26)
        (7-\offset, 37)
        (7-\offset, 25)
        (7-\offset, 20)
        (7-\offset, 43)
        (7-\offset, 39)
        (7-\offset, 16)
        (7-\offset, 18)
        (7-\offset, 50)
        (7-\offset, 42)
        (7-\offset, 41)
        (7-\offset, 64)
        (7-\offset, 65)
    };
\addlegendentry{6 reductions}
\pgfmathsetmacro{\offset}{7*\baseoffset}  % Reduction=7
\addplot+[only marks, mark=square, green!50!black]
    coordinates {
        (4-\offset, 4)
        (4-\offset, 5)
        (4-\offset, 6)
        (4-\offset, 3)
        (4-\offset, 2)
        (5-\offset, 9)
        (5-\offset, 8)
        (5-\offset, 10)
        (5-\offset, 7)
        (5-\offset, 6)
        (5-\offset, 12)
        (5-\offset, 5)
        (5-\offset, 4)
        (5-\offset, 16)
        (5-\offset, 3)
        (6-\offset, 18)
        (6-\offset, 15)
        (6-\offset, 16)
        (6-\offset, 12)
        (6-\offset, 20)
        (6-\offset, 17)
        (6-\offset, 14)
        (6-\offset, 13)
        (6-\offset, 11)
        (6-\offset, 10)
        (6-\offset, 24)
        (6-\offset, 8)
        (6-\offset, 9)
        (6-\offset, 21)
        (6-\offset, 19)
        (6-\offset, 6)
        (6-\offset, 32)
        (7-\offset, 36)
        (7-\offset, 30)
        (7-\offset, 32)
        (7-\offset, 24)
        (7-\offset, 40)
        (7-\offset, 34)
        (7-\offset, 28)
        (7-\offset, 29)
        (7-\offset, 26)
        (7-\offset, 27)
        (7-\offset, 22)
        (7-\offset, 25)
        (7-\offset, 20)
        (7-\offset, 21)
        (7-\offset, 48)
        (7-\offset, 18)
        (7-\offset, 16)
        (7-\offset, 35)
        (7-\offset, 33)
        (7-\offset, 31)
        (7-\offset, 42)
        (7-\offset, 23)
        (7-\offset, 15)
        (7-\offset, 38)
        (7-\offset, 12)
        (7-\offset, 49)
        (7-\offset, 37)
        (7-\offset, 41)
        (7-\offset, 64)
    };
\addlegendentry{7 reductions}
%\addplot+[only marks, mark=circle, thick, black!50!white]
%    coordinates {
%       (5-2*\baseoffset, 20)
%        (6-2*\baseoffset, 32)
%        };
%\addlegendentry{Section~\ref{sec:casestudies}}
\addplot+[only marks, mark=square*, black]     coordinates { (2,2)};
\addlegendentry{Paterson-Stockmeyer \cite{Paterson:1973:OnTheNumber} }

\draw[very thick,black, line width=7pt] (axis cs:1,0) -- (axis cs:1,2);
\draw[very thick,black, line width=7pt] (axis cs:2,0) -- (axis cs:2,4);
\draw[very thick,black, line width=7pt] (axis cs:3,0) -- (axis cs:3,6);
\draw[very thick,black, line width=7pt] (axis cs:4,0) -- (axis cs:4,9);
\draw[very thick,black, line width=7pt] (axis cs:5,0) -- (axis cs:5,12);
\draw[very thick,black, line width=7pt] (axis cs:6,0) -- (axis cs:6,16);
\draw[very thick,black, line width=7pt] (axis cs:7,0) -- (axis cs:7,20);
% \addplot[domain=3:7.5, samples=100, smooth, thick, color=blue] {x^2 - 1};

\addplot[only marks, mark=square, thick, black!50!white]     
coordinates { 
(4-1*\baseoffset,12)
(5-2*\baseoffset,20)
(6-3*\baseoffset,32)
(6-3*\baseoffset,30)
(7-5*\baseoffset,42)
%(7-4*\baseoffset,45)
};
\addlegendentry{Section~\ref{sec:casestudies}};

        \foreach \m in {3,4,5,6,7} {
            \addplot[domain=0:7, samples=11, smooth, thick, color=blue] 
                ({\m - \baseoffset * x}, {\m^2 - 1 - x});
        }

\addlegendentry{dof limit: $m^2-r-1$};

%\addplot+[only marks, mark=circle, black!50!white]
%    coordinates {
%       (5-2*\baseoffset, 20)
%        (6-2*\baseoffset, 32)
%        };
        

